Courcelle's Theorem Made Dynamic

Dynamic complexity is concerned with updating the output of a problem when the input is slightly changed. We study the dynamic complexity of model checking a fixed monadic second-order formula over evolving subgraphs of a fixed maximal graph having bounded tree-width; here the subgraph evolves by losing or gaining edges (from the maximal graph). We show that this problem is in DynFO (with LOGSPACE precomputation), via a reduction to a Dyck reachability problem on an acyclic automaton.

==> overall.tex <==
In this section, we analyze the complexity of our dynamic algorithm.
While adequate notions of reduction do exist in dynamic complexity
  (see e.g.~\cite{PI97,HI02}),
  our reduction does not satisfy all criteria, so we need to compute
  the complexity of our algorithm by hand.

First, denoting by $\calV$ and $\calL$ the vertex set and the label
set of $\Gamma_G$, Lemma~\ref{lem:Dyck} states that the Dyck reachability
problem in $\Gamma_G$ can be solved by using \FO update formulas
\emph{over the universe $\calV \uplus \calL$}.
However, we need \FO formulas over the universe~$V$ of our
\MSO model checking problem, i.e., $V$~is the vertex set of the input graph.
Hence, we must embed $\calV \uplus \calL$ into a set of tuples
of elements of~$V$ of finite arity.

Lemma~\ref{lemma:puredecomposition} states that $\mathcal{T}_\star$ is of
height at most $c(\kappa) \cdot (\log_2(N)+1)$, where $N = |V|$, and
Lemma~\ref{lem:progression} proves that
$|\calS_i| \leqslant 2 c(\kappa) \cdot (\log_2(N)+1)$ for all $i \leqslant N$.
It follows that $|\calV| = 1 + \sum_{i=0}^N |Q|^{|\calS_i|} =
\calO(N^{2 c(\kappa) \log_2(|Q|) + 1})$, which is
polynomial in~$|V|$. Likewise, $|\calL|$~is polynomial in~$|V|$, and
therefore $\calV \uplus \calL$ can be embedded into some set~$V^k$,
where $k$ is a large enough integer (which depends only on~$\kappa$
and on the \MSO formula~$\varphi$).

In the end, during the precomputation phase, 
the algorithm successively computes:
\begin{enumerate}
\item a binary rooted tree decomposition $\mathcal{D}_\star =
  \tuple{\mathcal{T}_\star,\mathbf{T}_{\star}}$ of the maximal
  graph $G_\star = \tuple{V,E_\star}$, of width $4\kappa+3$,
  such as described in Lemma~\ref{lemma:puredecomposition};
\item a (bottom-up, deterministic) tree automaton
$\calA_{\varphi,4\kappa+3}$ such as defined in Courcelle's theorem;
\item a $\calD_\star$-coloring function $\chi$, a $(\chi,\calD_\star)$-succinct tree
  decomposition of $G_\star$, and a bottom-up progression
  $(\calS_i)_{0 \leqslant i \leqslant N}$ of $\calT_\star$;
\item the vertices, labels and edges of the graph~$\Gamma_{G_E}$,
where $G_E$ is the initial input graph;
\item an embedding $\calV \uplus \calL \mapsto V^k$;
\item mappings $e \mapsto i$, $(e,\gamma) \mapsto \add_e(\gamma)$
and $(e,\gamma) \mapsto \del_e(\gamma)$ mentioned in the proof of
Proposition~\ref{pro:small-change};
\item the value of the auxiliary predicate $\Delta$
(mentioned in Lemma~\ref{lem:Dyck}) on
$\Gamma_{G_E}$.
\end{enumerate}

\begin{lem}
\label{lem:precomputation-in-logspace}
Each of these 7 steps can be performed in \LOGSPACE.
\end{lem}

\begin{proof}
The formula $\varphi$ and the integer~$\kappa$ are fixed.
Hence, Lemma~\ref{lemma:puredecomposition} proves that the step~1 can be
performed in \LOGSPACE, and the step~2 is completed in constant time.
Since performing the steps~3--6 in \LOGSPACE is straightforward,
it remains to deal with the step~7.

Let $\varpi$ be a path with label $\lambda$ in $\Gamma_G$.
We say that $\varpi$ is a \emph{Dyck prefix} path
if $\lambda$ is a prefix of a Dyck word (which may be $\lambda$ itself)
and if its proper prefixes are not Dyck words;
that $\varpi$ is a \emph{Dyck suffix} path
if $\lambda$ is a suffix of a Dyck word
and if its proper suffixes are not Dyck words;
that $\varpi$ is a \emph{minimal Dyck} path if
$\varpi$ is both a Dyck prefix and a Dyck suffix path.

Minimal non-empty Dyck paths are paths of the form
$(i-1) \xrightarrow{\bullet} (i-1,\gamma)$, $(\ell,\pi) \xrightarrow{\bullet} \top$,
and $(i-1,\pi) \xrightarrow{(i-1,\pi)^+} (i-1) \xrightarrow{\bullet}
(i-1,\gamma) \xrightarrow{(i-1,\pi)^-} (i,\pi')$.
Since Dyck prefix paths are the prefixes of minimal Dyck paths,
and Dyck suffix paths are the suffixes of minimal Dyck paths,
they have length at most 2.
Furthermore, every Dyck path is a product of non-empty minimal Dyck paths.
In addition, if $\varpi_1$ and $\varpi_2$ are paths with labels
$\lambda_1$ and $\lambda_2$ such that $\lambda_1 \cdot \lambda_2$
is a Dyck word, then there exists factorisations
$\varpi_1 = \varpi_1^{\INIT} \cdot \varpi_1^{\END}$ and
$\varpi_2 = \varpi_2^{\INIT} \cdot \varpi_2^{\END}$ such that
$\varpi_1^{\INIT}$ and $\varpi_2^{\END}$ are Dyck paths,
$\varpi_1^{\END}$ is a Dyck prefix and $\varpi_2^{\INIT}$ is a Dyck suffix.

Hence, the predicate $\Delta(x_1,y_1,x_2,y_2)$ holds if, and only~if,
there exists vertices $z_1$ and~$z_2$ and paths~$\varpi_1$ (from~$z_1$ to~$y_1$)
and $\varpi_2$ (from~$x_2$ to~$z_2$) with labels $\lambda_1$ and~$\lambda_2$ such that:
\begin{itemize}
 \item $\varpi_1$ and $\varpi_2$ are of length at most 2,
 and $\lambda_1 \cdot \lambda_2$ is a Dyck word;
 \item there exists Dyck paths from $x_1$ to $z_1$ and from $z_2$ to $y_2$.
\end{itemize}
Finally, note that every vertex of $\Gamma_G$ is the source of at most
one minimal Dyck path. Consequently, for any two vertices~$x$ and~$y$
of~$\Gamma_G$, checking if there exists a Dyck path from~$x$ to~$y$
can be done in \LOGSPACE, and $\Delta$ can be computed in \LOGSPACE
too.
\end{proof}

We sum up the above results as follows.
First, we perform a \LOGSPACE precomputation,
and construct a graph $\Gamma_G$ whose vertex, label and edge sets
can be represented as predicates of finite arity on the universe $V$.
Then, during the update phases, whenever introducing or deleting an
edge $e$ in $G$, we replace one edge of $\Gamma_G$ by another one,
and these edges are identified by precomputed \FO formulas taking the
edge $e$ into account, as stated in Proposition~\ref{pro:small-change}.
Consequently, and since the Dyck reachability problem is in \Dyn\FO,
updating the edge-membership predicate
of $\Gamma_G$ and the auxiliary predicate $\Delta$,
which is useful for solving the Dyck reachability problem in $\Gamma_G$,
can be done with \FO formulas.
Finally, deciding whether $G$ satisfies the formula $\varphi$,
i.e., whether there exists a suitable Dyck path in $\Gamma_G$,
can be done using directly the auxiliary predicate $\Delta$,
which completes the proof of Theorem~\ref{mainresult}.

